Quantum computing, phase estimation and applications

In this thesis, attention is paid to small experimental testbed applications with respect to the quantum phase estimation algorithm, the core approach for finding energy eigenvalues. An iterative scheme for quantum phase estimation (IPEA) is derived from the Kitaev phase estimation, a study of robustness of the IPEA utilized as a few-qubit testbed application is performed, and an improved protocol for phase reference alignment is presented. Additionally, a short overview of quantum cryptography is given, with a particular focus on quantum steganography and authentication.

==> 00_dedication.tex <==
\newpage
\vglue 6cm 
\centerline{\bf Dedication}
\vglue 2cm 
%It is very pleasant if you dedicate this piece of work to someone 
%who you especially like or who likes you.

\begin{center}
%{\em To humankind}.

%Do not become attached to the things you like,

%do not maintain aversion to the things you dislike.

%Sorrow, fear and bondage come from one's likes and
%dislikes.
\end{center}

% or {\em To my parents},  

% or something similar.



==> state-of-the-art.tex <==
%---------------------------------------------------------%
% Chapter: State of the Art                               %
%---------------------------------------------------------%


State of the art, algoritmy (gate model, adiabatický a měřící model), kryptografie, technologie, výhled, senzory

 - v téhle kapitole by mělo vyplinout proč se v dalším textu budu zabývat právě PEA a krypto

